Towards Efficient and Domain-Agnostic Evasion Attack with High-dimensional Categorical Inputs

Our work targets at searching feasible adversarial perturbation to attack a classifier with high-dimensional categorical inputs in a domain-agnostic setting. This is intrinsically an NP-hard knapsack problem where the exploration space becomes explosively larger as the feature dimension increases. Without the help of domain knowledge, solving this problem via heuristic method, such as Branch-and-Bound, suffers from exponential complexity, yet can bring arbitrarily bad attack results. We address the challenge via the lens of multi-armed bandit based combinatorial search. Our proposed method, namely FEAT, treats modifying each categorical feature as pulling an arm in multi-armed bandit programming. Our objective is to achieve highly efficient and effective attack using an Orthogonal Matching Pursuit (OMP)-enhanced Upper Confidence Bound (UCB) exploration strategy. Our theoretical analysis bounding the regret gap of FEAT guarantees its practical attack performance. In empirical analysis, we compare FEAT with other state-of-the-art domain-agnostic attack methods over various real-world categorical data sets of different applications. Substantial experimental observations confirm the expected efficiency and attack effectiveness of FEAT applied in different application scenarios. Our work further hints the applicability of FEAT for assessing the adversarial vulnerability of classification systems with high-dimensional categorical inputs.

==> 7_checklist.tex <==
\newpage
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please read the checklist guidelines carefully for information on how to answer these questions.  For each question, change the default \answerTODO{} to \answerYes{}, \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf justification to your answer}, either by referencing the appropriate section of your paper or providing a brief inline description.  For example:
%\begin{itemize}
%  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
 % \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your answers.  Note that the Checklist section does not count towards the page limit.  In your paper, please delete this instructions block and only keep the Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
  \answerYes{See Abstract and Section 1.}  %\answerTODO{} 
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes % \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo % \answerTODO{}
  \item Did you describe the limitations of your work?
     \answerNo{} %\answerTODO{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
   \answerYes{We state the assumptions of all theoretical results in section 4}
 \item Did you include complete proofs of all theoretical results?
   \answerYes{We report the complete proofs of all theoretical results in the Appendix.} %\answerTODO{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We provide core codes as a URL.} % \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
   \answerYes{Experimental training  details are at Section 5.1}  % \answerTODO{}
 \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
   \answerNA{}  % \answerTODO{}
 \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    % \answerTODO{}
    \answerYes{{The total amount and the type of computing resource used in our experiments are described in Section 5.1}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    % \answerTODO{}
    \answerYes{{Citations for the existing assets (code, data and baseline models) are provided in Section 5.2}}
  \item Did you mention the license of the assets?
%    \answerTODO{} \FJ{I am not sure what this means. }
\answerYes{We mentioned relevant licenses when we introduce respective codes and data.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We include new codes in this work as a URL.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{These data are publicly available and have been frequently used for research purposes.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    % \answerTODO{}
    \answerNo{There are no personally identifiable information or offensive content in our discussion .}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> Table.tex <==

\begin{table}[]
\linespread{2.0}
\begin{tabular}{cc}
\hline
\textbf{Attack Method} & \textbf{The number of times the decision confidence of $f$ is evaluated} \\ \hline
FSGS                   &   $\sum_{t = 0}^T((N-t)*M*2^t)$                                                                       \\ \hline
GradAttack             & $T*\sum_{k = 0}^K(C^k_K*M^k)$                                                                          \\ \hline
OMPGS                  & $\sum_{t = 0}^T(K*2^t)$                                                                          \\ \hline
\textbf{FEAT-B}        &  $\mathbf{N}*\mathbf{M} + \mathbf{T}$                                                                        \\ \hline
\textbf{FEAT}          &  $(\mathbf{K}*\mathbf{M} + \mathbf{\tau})*\mathbf{T}$                                                                        \\ \hline
\end{tabular}
\end{table}


\begin{table*}[]

\begin{tabular}{|c|cccc||cccc|}
\hline
\multirow{2}{*}{\textbf{Yelp-5}} & \multicolumn{4}{c||}{\textbf{Budget = 6}}                                                                                                                & \multicolumn{4}{c|}{\textbf{Budget = 8}}                                                                                                                \\ \cline{2-9} 
                                  & \multicolumn{1}{c|}{\textbf{AC}} & \multicolumn{1}{c|}{\textbf{AT}} & \multicolumn{1}{c|}{\textbf{AE}} & \textbf{SR}  & \multicolumn{1}{c|}{\textbf{AC}} & \multicolumn{1}{c|}{\textbf{AT}} & \multicolumn{1}{c|}{\textbf{AE}} & \textbf{SR} \\ \hline
FSGS                            & \multicolumn{1}{c|}{1.61}        & \multicolumn{1}{c|}{0.52}        & \multicolumn{1}{c|}{23000}       & 0.97                & \multicolumn{1}{c|}{1.63}        & \multicolumn{1}{c|}{1.62}        & \multicolumn{1}{c|}{84000}       & 0.95        \\ \hline
GradAttack                      & \multicolumn{1}{c|}{5.08}        & \multicolumn{1}{c|}{0.08}        & \multicolumn{1}{c|}{42000}         & 0.61               & \multicolumn{1}{c|}{6.75}        & \multicolumn{1}{c|}{0.12}       & \multicolumn{1}{c|}{50000}         & 0.76        \\ \hline
OMPGS                           & \multicolumn{1}{c|}{1.95}        & \multicolumn{1}{c|}{1.25}        & \multicolumn{1}{c|}{7000}        & 0.96              & \multicolumn{1}{c|}{1.95}        & \multicolumn{1}{c|}{0.82}        & \multicolumn{1}{c|}{7000}        & 0.96        \\ \hline
TextBugger                      & \multicolumn{1}{c|}{3.29}        & \multicolumn{1}{c|}{1.18}        & \multicolumn{1}{c|}{23}          & 0.64                & \multicolumn{1}{c|}{4.04}        & \multicolumn{1}{c|}{1.43}        & \multicolumn{1}{c|}{28}          & 0.75        \\ \hline
TextFooler                      & \multicolumn{1}{c|}{1.37}        & \multicolumn{1}{c|}{0.19}        & \multicolumn{1}{c|}{152}         & 0.86                 & \multicolumn{1}{c|}{1.37}        & \multicolumn{1}{c|}{0.19}        & \multicolumn{1}{c|}{152}         & 0.86        \\ \hline
\textbf{FEAT-B}                  & \multicolumn{1}{c|}{\textbf{2.11}}        & \multicolumn{1}{c|}{\textbf{0.13}}       & \multicolumn{1}{c|}{\textbf{2000}}        & \textbf{0.90}              & \multicolumn{1}{c|}{\textbf{2.22}}        & \multicolumn{1}{c|}{\textbf{0.13}}        & \multicolumn{1}{c|}{\textbf{2000}}        & \textbf{0.92}        \\ \hline
\textbf{FEAT}                   & \multicolumn{1}{c|}{\textbf{2.56}}        & \multicolumn{1}{c|}{\textbf{0.14}}        & \multicolumn{1}{c|}{\textbf{643}}         & \textbf{0.96}               & \multicolumn{1}{c|}{\textbf{2.20}}        & \multicolumn{1}{c|}{\textbf{0.12}}        & \multicolumn{1}{c|}{\textbf{883}}         & \textbf{0.97}       \\ \hline
\end{tabular}
\end{table*}


% \begin{table}[]
% \resizebox{1\linewidth}{!}{
% \begin{tabular}{ccccccccc}
% \toprule
% \multirow{2}{*}{\textbf{Yelp-5}} & \multicolumn{4}{c}{\textbf{Budget = 6}}                       & \multicolumn{4}{c}{\textbf{Budget = 8}}                       \\ \cline{2-9} 
%                                  & \textbf{AC} $\downarrow$   & \textbf{AT} $\downarrow$   & \textbf{AE} $\downarrow$   & \textbf{SR} $\uparrow$   & \textbf{AC} $\downarrow$   & \textbf{AT} $\downarrow$   & \textbf{AE} $\downarrow$   & \textbf{SR} $\uparrow$   \\ \hline
% FSGS                             & 1.61          & 0.52          & 23000         & 0.97          & 1.63          & 1.62          & 84000         & 0.95          \\ \hline
% GradAttack                       & 5.08          & 0.08          & 42000         & 0.61          & 6.75          & 0.12          & 50000         & 0.76          \\ \hline
% OMPGS                            & 1.95          & 1.25          & 7000          & 0.96          & 1.95          & 0.82          & 7000          & 0.96          \\ \hline
% TextBugger                       & 3.29          & 1.18          & 23            & 0.64          & 4.04          & 1.43          & 28            & 0.75          \\ \hline
% TextFooler                       & 1.37          & 0.19          & 152           & 0.86          & 1.37          & 0.19          & 152           & 0.86          \\ \hline
% \textbf{FEAT-B}                  & \textbf{2.11} & \textbf{0.13} & \textbf{2000} & \textbf{0.90} & \textbf{2.22} & \textbf{0.13} & \textbf{2000} & \textbf{0.92} \\ \hline
% \textbf{FEAT}                    & \textbf{2.56} & \textbf{0.14} & \textbf{643}  & \textbf{0.96} & \textbf{2.20} & \textbf{0.12} & \textbf{883}  & \textbf{0.97} \\ 
% \bottomrule
% \end{tabular}
% }
% \end{table}


\begin{table*}[]
\renewcommand{\arraystretch}{1.2}
\resizebox{1\linewidth}{!}{
\begin{tabular}{ccccccccc}
\toprule
\multirow{2}{*}{\textbf{Yelp-5}} & \multicolumn{4}{c}{\textbf{Budget = 6}}                       & \multicolumn{4}{c}{\textbf{Budget = 8}}                       \\ \cline{2-9} 
                                 & \textbf{AT} $\downarrow$   & \textbf{AE} $\downarrow$   & \textbf{AC} $\downarrow$   & \textbf{SR} $\uparrow$   & \textbf{AT} $\downarrow$   & \textbf{AE} $\downarrow$   & \textbf{AC} $\downarrow$   & \textbf{SR} $\uparrow$   \\ \hline
FSGS                             & 0.52          & 23000         & 1.61          & 0.97          & 1.63          & 84000         & 1.63          & 0.95          \\ \hline
GradAttack                       & 0.08          & 42000         & 5.08          & 0.61          & 6.75          & 50000         & 6.75          & 0.76          \\ \hline
OMPGS                            & 1.25          & 7000          & 1.95          & 0.96          & 1.95          & 7000          & 1.95          & 0.96          \\ \hline
TextBugger                       & 1.18          & 23            & 3.29          & 0.64          & 4.04          & 28            & 4.04          & 0.75          \\ \hline
TextFooler                       & 0.19          & 152           & 1.37          & 0.86          & 1.37          & 152           & 1.37          & 0.86          \\ \hline
\textbf{FEAT-B}                  & \textbf{0.13} & \textbf{2000} & \textbf{2.11} & \textbf{0.90} & \textbf{2.22} & \textbf{2000} & \textbf{2.22} & \textbf{0.92} \\ \hline
\textbf{FEAT}                    & \textbf{0.14} & \textbf{643}  & \textbf{2.56} & \textbf{0.96} & \textbf{2.20} & \textbf{883}  & \textbf{2.20} & \textbf{0.97} \\ \bottomrule
\end{tabular}
}
\end{table*}


\begin{table*}[]
\renewcommand{\arraystretch}{1.2}
\resizebox{1\linewidth}{!}{
\begin{tabular}{ccccccccc}
\toprule
\multirow{2}{*}{\textbf{IPS}} & \multicolumn{4}{c}{\textbf{Budget = 5}}                        & \multicolumn{4}{c}{\textbf{Budget = 6}}                        \\ \cline{2-9} 
                              & \textbf{AT} $\downarrow$   & \textbf{AE} $\downarrow$   & \textbf{AC} $\downarrow$   & \textbf{SR} $\uparrow$   & \textbf{AT} $\downarrow$   & \textbf{AE} $\downarrow$   & \textbf{AC} $\downarrow$   & \textbf{SR} $\uparrow$   \\ \hline
FSGS                          & 136            & 37000         & 1.22          & 0.80          & 56.15          & 70000         & 1.41          & 0.85          \\ \hline
GradAttack                    & 21.15          & 2100          & 1.76          & 0.59          & 23.67          & 2500          & 1.9           & 0.61          \\ \hline
OMPGS                         & 1.99           & 127           & 2.19          & 0.77          & 0.99           & 92.09         & 1.9           & 0.83          \\ \hline
\textbf{FEAT-B}               & \textbf{19.52} & \textbf{2500} & \textbf{1.25} & \textbf{0.64} & \textbf{19.49} & \textbf{2800} & \textbf{1.4}  & \textbf{0.65} \\ \hline
\textbf{FEAT}                 & \textbf{0.28}  & \textbf{111}  & \textbf{4.66} & \textbf{0.92} & \textbf{0.28}  & \textbf{121}  & \textbf{5.07} & \textbf{0.94} \\ \bottomrule
\end{tabular}
}
\end{table*}

\begin{table*}[]
\renewcommand{\arraystretch}{1.2}
\resizebox{1\linewidth}{!}{
\begin{tabular}{ccccccccc}
\toprule
\multirow{2}{*}{\textbf{EHR}} & \multicolumn{4}{c}{\textbf{Budget = 4}}                         & \multicolumn{4}{c}{\textbf{Budget = 6}}                          \\ \cline{2-9} 
                             & \textbf{AT} $\downarrow$   & \textbf{AE} $\downarrow$   & \textbf{AC} $\downarrow$   & \textbf{SR} $\uparrow$   & \textbf{AT} $\downarrow$   & \textbf{AE} $\downarrow$   & \textbf{AC} $\downarrow$   & \textbf{SR} $\uparrow$   \\ \hline
FSGS                          & 446             & 58000         & 1.65          & 0.84          & 482             & 58000         & 1.65          & 0.84           \\ \hline
GradAttack                    & 0.06            & 4             & 2             & 0.63          & 0.062           & 4.30          & 2             & 0.62           \\ \hline
OMPGS                         & 30.01           & 35.18         & 2             & 0.94          & 27.5            & 35            & 2             & 0.94           \\ \hline
\textbf{FEAT-B}               & \textbf{107.39} & \textbf{5000} & \textbf{4.32} & \textbf{0.37} & \textbf{106.45} & \textbf{5000} & \textbf{4.34} & \textbf{0.382} \\ \hline
\textbf{FEAT}                 & \textbf{0.74}   & \textbf{55}   & \textbf{3.83} & \textbf{0.93} & \textbf{0.35}   & \textbf{20}   & \textbf{5.13} & \textbf{0.94}  \\ \bottomrule
\end{tabular}
}
\end{table*}



\begin{table*}[]
\renewcommand{\arraystretch}{1.2}
\resizebox{1\linewidth}{!}{
\begin{tabular}{ccccccccc}
\toprule
\multirow{2}{*}{\textbf{PEDec}} & \multicolumn{4}{c}{\textbf{Budget = 10}}                      & \multicolumn{4}{c}{\textbf{Budget = 12}}                       \\ \cline{2-9} 
                                & \textbf{AT} $\downarrow$   & \textbf{AE} $\downarrow$   & \textbf{AC} $\downarrow$   & \textbf{SR} $\uparrow$   & \textbf{AT} $\downarrow$   & \textbf{AE} $\downarrow$   & \textbf{AC} $\downarrow$   & \textbf{SR} $\uparrow$   \\ \hline
FSGS                            & 277           & 39000         & 3.74          & 0.94          & 310           & 41000         & 3.79           & 0.95          \\ \hline
GradAttack                      & 0.07          & 28            & 6.11          & 0.51          & 0.08          & 32            & 6.87           & 0.60          \\ \hline
OMPGS                           & 219           & 7400          & 6.39          & 0.73          & 594           & 20000         & 7.21           & 0.81          \\ \hline
\textbf{FEAT-B}                 & \textbf{6.51} & \textbf{2200} & \textbf{7.64} & \textbf{0.70} & \textbf{6.78} & \textbf{2100} & \textbf{8.19}  & \textbf{0.83} \\ \hline
\textbf{FEAT}                   & \textbf{3.51} & \textbf{7000} & \textbf{9.43} & \textbf{0.72} & \textbf{3.14} & \textbf{6600} & \textbf{10.99} & \textbf{0.87} \\ \bottomrule
\end{tabular}
}
\end{table*}








\begin{table}[]
\begin{tabular}{|c|cccc||cccc|}
\hline
 & \multicolumn{4}{c||}{  \textbf{Budget = 10}}                                                                                                                                                                                                           & \multicolumn{4}{c|}{  \textbf{Budget = 12}}                                                                                                                                                                                                           \\ \cline{2-9} 
\multirow{-2}{*}{ \textbf{PEDec}} & \multicolumn{1}{c|}{  \textbf{AC}} & \multicolumn{1}{c|}{  \textbf{AT}} & \multicolumn{1}{c|}{  \textbf{AE}} &   \textbf{SR} & \multicolumn{1}{c|}{  \textbf{AC}} & \multicolumn{1}{c|}{  \textbf{AT}} & \multicolumn{1}{c|}{  \textbf{AE}} &   \textbf{SR} \\ \hline

{  FSGS}                    & \multicolumn{1}{c|}{  3.74}       & \multicolumn{1}{c|}{  277}      & \multicolumn{1}{c|}{39000}       & {0.94}       & \multicolumn{1}{c|}{  3.79}       & \multicolumn{1}{c|}{  310}     & \multicolumn{1}{c|}{ 41000}       & {0.95}       \\ \hline

{  GradAttack}              & \multicolumn{1}{c|}{  6.11}       & \multicolumn{1}{c|}{  0.07}      & \multicolumn{1}{c|}{  28}        & {  0.51}          & \multicolumn{1}{c|}{  6.87}       & \multicolumn{1}{c|}{  0.08}      & \multicolumn{1}{c|}{  32}       & {  0.60}          \\ \hline

{  OMPGS}                   & \multicolumn{1}{c|}{  6.39}       & \multicolumn{1}{c|}{ 219}      & \multicolumn{1}{c|}{ 7400}       & {  0.73}        & \multicolumn{1}{c|}{  7.21}       & \multicolumn{1}{c|}{ 594}         & \multicolumn{1}{c|}{20000}       & {0.81}       \\ \hline

{\textbf{FEAT-B}}                   & \multicolumn{1}{c|}{\textbf{  7.64}}       & \multicolumn{1}{c|}{\textbf{  6.51}}       & \multicolumn{1}{c|}{\textbf{ 2200}}       & \textbf{  0.70}        & \multicolumn{1}{c|}{\textbf{  8.19}}       & \multicolumn{1}{c|}{\textbf{  6.78}}       & \multicolumn{1}{c|}{\textbf{2100}}       & \textbf{0.83}         \\ \hline

{  \textbf{FEAT}}           & \multicolumn{1}{c|}{\textbf{  9.43}}       & \multicolumn{1}{c|}{\textbf{  3.51}}        & \multicolumn{1}{c|}{\textbf{7000}}       & \textbf{0.72}        & \multicolumn{1}{c|}{\textbf{  10.99}}       & \multicolumn{1}{c|}{\textbf{  3.14}}       & \multicolumn{1}{c|}{\textbf{  6600}}        & \textbf{ 0.87}        \\ \hline
\end{tabular}
\end{table}

















\begin{table}[]
\begin{tabular}{|c|cccc||cccc|}
\hline
 & \multicolumn{4}{c||}{   \textbf{Budget = 4}}   & \multicolumn{4}{c|}{   \textbf{Budget = 6}}        \\ \cline{2-9} 

\multirow{-2}{*}{   \textbf{EHR}} & \multicolumn{1}{c|}{   \textbf{AC}} & \multicolumn{1}{c|}{   \textbf{AT}} & \multicolumn{1}{c|}{   \textbf{AE}} &    \textbf{SR} & \multicolumn{1}{c|}{   \textbf{AC}}                  & \multicolumn{1}{c|}{   \textbf{AT}} & \multicolumn{1}{c|}{   \textbf{AE}} &    \textbf{SR} \\ \hline

{   FSGS}                           & \multicolumn{1}{c|}{   1.65}        & \multicolumn{1}{c|}{   446}         & \multicolumn{1}{c|}{58000}        & {   0.84}       & \multicolumn{1}{c|}{   1.65} & \multicolumn{1}{c|}{   482}         & \multicolumn{1}{c|}{58000 }        & {   0.84}       \\ \hline

{   GradAttack}                     & \multicolumn{1}{c|}{   2}           & \multicolumn{1}{c|}{   0.06}       & \multicolumn{1}{c|}{4}       & {0.63}           & \multicolumn{1}{c|}{   2}                            & \multicolumn{1}{c|}{   0.062}      & \multicolumn{1}{c|}{   4.30}       & {   0.62}       \\ \hline

{   OMPGS}                          & \multicolumn{1}{c|}{   2}           & \multicolumn{1}{c|}{   30.01}       & \multicolumn{1}{c|}{  35.18}        &    0.94      & \multicolumn{1}{c|}{   2}                            & \multicolumn{1}{c|}{   27.5}        & \multicolumn{1}{c|}{ 35}        &    0.94          \\ \hline

{\textbf{FEAT-B}}                          & \multicolumn{1}{c|}{   4.32}       & \multicolumn{1}{c|}{   107.39}     & \multicolumn{1}{c|}{5000}       & \textbf{ 0.37}     & \multicolumn{1}{c|}{   4.34}                        & \multicolumn{1}{c|}{   106.45}      & \multicolumn{1}{c|}{5000}       & \textbf{0.382}     \\ \hline

{   \textbf{FEAT}}                  & \multicolumn{1}{c|}{ 3.83}       & \multicolumn{1}{c|}{0.74}      & \multicolumn{1}{c|}{ 55}       & \textbf{ 0.93}       & \multicolumn{1}{c|}{   5.13}                       & \multicolumn{1}{c|}{   0.35}       & \multicolumn{1}{c|}{  20}       & \textbf{ 0.94}          \\ \hline
\end{tabular}

\end{table}



\begin{table}[]
\begin{tabular}{|c|cccc||cccc|}
\toprule
% \hline
\multirow{2}{*}{\textbf{IPS} } & \multicolumn{4}{c||}{\textbf{Budget = 5}}                                                                                                                & \multicolumn{4}{c|}{\textbf{Budget = 6}}                                                                                                                \\ \cline{2-9} 
                              & \multicolumn{1}{c|}{\textbf{AC} $\downarrow$} & \multicolumn{1}{c|}{\textbf{AT}} & \multicolumn{1}{c|}{\textbf{AE}} & \textbf{SR}  & \multicolumn{1}{c|}{\textbf{AC}} & \multicolumn{1}{c|}{\textbf{AT}} & \multicolumn{1}{c|}{\textbf{AE}} & \textbf{SR} \\ \hline
FSGS                            & \multicolumn{1}{c|}{1.22}        & \multicolumn{1}{c|}{136}         & \multicolumn{1}{c|}{37000}       & 0.80         & \multicolumn{1}{c|}{1.41}        & \multicolumn{1}{c|}{56.15}         & \multicolumn{1}{c|}{70000}       & 0.85        \\ \hline
GradAttack                      & \multicolumn{1}{c|}{1.76}        & \multicolumn{1}{c|}{21.15}        & \multicolumn{1}{c|}{2100}        & 0.59             & \multicolumn{1}{c|}{1.9}         & \multicolumn{1}{c|}{23.67}       & \multicolumn{1}{c|}{2500}        & 0.61        \\ \hline
OMPGS                            & \multicolumn{1}{c|}{2.19}        & \multicolumn{1}{c|}{1.99}        & \multicolumn{1}{c|}{127}          & 0.77          & \multicolumn{1}{c|}{1.9}         & \multicolumn{1}{c|}{0.99}        & \multicolumn{1}{c|}{92.09}          & 0.83        \\ \hline
\textbf{FEAT-B}                         & \multicolumn{1}{c|}{\textbf{1.25}}        & \multicolumn{1}{c|}{\textbf{19.52}}       & \multicolumn{1}{c|}{\textbf{2500}}       & \textbf{0.64}        & \multicolumn{1}{c|}{\textbf{1.4}}         & \multicolumn{1}{c|}{\textbf{19.49}}       & \multicolumn{1}{c|}{\textbf{2800}}        & \textbf{0.65}        \\ \hline
\textbf{FEAT}                 & \multicolumn{1}{c|}{\textbf{4.66}}        & \multicolumn{1}{c|}{\textbf{0.28}}         & \multicolumn{1}{c|}{\textbf{111}}          & \textbf{0.92}        & \multicolumn{1}{c|}{\textbf{5.07}}        & \multicolumn{1}{c|}{\textbf{0.28}}        & \multicolumn{1}{c|}{\textbf{121}}          & \textbf{0.94}       \\ \hline
\end{tabular}
\end{table}




\begin{table*}[t]
\centering
%\caption{This is the attack results on IPS dataset with $T_L$ 3600 seconds.}
\label{tab:IPS performance}
\scriptsize
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{c|cccc|cccc}
\toprule
\multirow{2}{*}{\textbf{IPS}} & \multicolumn{4}{c}{ {Budget = 5}}                        & \multicolumn{4}{c}{ {Budget = 6}}                        \\ \cline{2-9} 
                              & \textbf{AT} $\downarrow$   & \textbf{AE} $\downarrow$   & \textbf{AC} $\downarrow$   & \textbf{SR} $\uparrow$   & \textbf{AT} $\downarrow$   & \textbf{AE} $\downarrow$   & \textbf{AC} $\downarrow$   & \textbf{SR} $\uparrow$   \\ \hline
FSGS                          & 136            & 37000         & 1.22          & 0.80          & 56.15          & 70000         & 1.41          & 0.85          \\ \hline
GradAttack                    & 21.15          & 2100          & 1.76          & 0.59          & 23.67          & 2500          & 1.9           & 0.61          \\ \hline
OMPGS                         & 1.99           & 127           & 2.19          & 0.77          & 0.99           & 92.09         & 1.9           & 0.83          \\ \hline
\textbf{FEAT-B}               & \textbf{19.52} & \textbf{2500} & \textbf{1.25} & \textbf{0.64} & \textbf{19.49} & \textbf{2800} & \textbf{1.4}  & \textbf{0.65} \\ \hline
\textbf{FEAT}                 & \textbf{0.28}  & \textbf{111}  & \textbf{4.66} & \textbf{0.92} & \textbf{0.28}  & \textbf{121}  & \textbf{5.07} & \textbf{0.94} \\ \bottomrule
\end{tabular}
}
\end{table*}



\begin{table}[]
\begin{tabular}{lllll}
TextBugger & sentence                                                                                                                                                                                                                                                                                  & original label with confidence & attacked label with confidence &  \\
TextBudder & "I hate this place. It's very loud, the service is very poor, and the food is so-so. \textbackslash{}\textbackslash If you want good Chinese in Pittsburgh, try China Palace (Shadyside) or Sesame Inn (Station Square or North Hills). They're quieter, with very good food \& service." &                                &                                &  \\
FEAT       &                                                                                                                                                                                                                                                                                           &                                &                                &  \\
           &                                                                                                                                                                                                                                                                                           &                                &                                & 
\end{tabular}
\end{table}
